Implicit Gaussian process representation of vector fields over arbitrary latent manifolds

Gaussian processes (GPs) are popular nonparametric statistical models for learning unknown functions and quantifying the spatiotemporal uncertainty in data. Recent works have extended GPs to model scalar and vector quantities distributed over non-Euclidean domains, including smooth manifolds appearing in numerous fields such as computer vision, dynamical systems, and neuroscience. However, these approaches assume that the manifold underlying the data is known, limiting their practical utility. We introduce RVGP, a generalisation of GPs for learning vector signals over latent Riemannian manifolds. Our method uses positional encoding with eigenfunctions of the connection Laplacian, associated with the tangent bundle, readily derived from common graph-based approximation of data. We demonstrate that RVGP possesses global regularity over the manifold, which allows it to super-resolve and inpaint vector fields while preserving singularities. Furthermore, we use RVGP to reconstruct high-density neural dynamics derived from low-density EEG recordings in healthy individuals and Alzheimer's patients. We show that vector field singularities are important disease markers and that their reconstruction leads to a comparable classification accuracy of disease states to high-density recordings. Thus, our method overcomes a significant practical limitation in experimental and clinical applications.

==> iclr2024_conference <==
\begin{thebibliography}{63}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Barbero et~al.(2022)Barbero, Bodnar, de~Ocáriz~Borde, Bronstein,
  Veličković, and Liò]{barbero2022sheaf}
Federico Barbero, Cristian Bodnar, Haitz~Sáez de~Ocáriz~Borde, Michael
  Bronstein, Petar Veličković, and Pietro Liò.
\newblock Sheaf neural networks with connection laplacians, 2022.

\bibitem[Battiloro et~al.(2023)Battiloro, Wang, Riess, Di~Lorenzo, and
  Ribeiro]{battiloro2023tangent}
Claudio Battiloro, Zhiyang Wang, Hans Riess, Paolo Di~Lorenzo, and Alejandro
  Ribeiro.
\newblock Tangent bundle convolutional learning: from manifolds to cellular
  sheaves and back.
\newblock \emph{arXiv preprint arXiv:2303.11323}, 2023.

\bibitem[Belkin \& Niyogi(2003)Belkin and Niyogi]{Belkin2003}
Mikhail Belkin and Partha Niyogi.
\newblock {Laplacian eigenmaps for dimensionality reduction and data
  representation}.
\newblock \emph{Neural Comput.}, 15\penalty0 (6):\penalty0 1373--1396, 2003.
\newblock ISSN 08997667.
\newblock \doi{10.1162/089976603321780317}.

\bibitem[Berger(1934)]{berger1934elektrenkephalogramm}
Hans Berger.
\newblock {\"U}ber das elektrenkephalogramm des menschen.
\newblock \emph{DMW-Deutsche Medizinische Wochenschrift}, 60\penalty0
  (51):\penalty0 1947--1949, 1934.

\bibitem[Berline~N.(1996)]{berline}
Vergne~M. Berline~N., Getzler~E.
\newblock \emph{Heat kernels and Dirac operators}.
\newblock Springer, 2nd. edition, 1996.

\bibitem[Besthorn et~al.(1994)Besthorn, F{\"o}rstl, Geiger-Kabisch, Sattel,
  Gasser, and Schreiter-Gasser]{besthorn1994eeg}
Christoph Besthorn, Hans F{\"o}rstl, Claudia Geiger-Kabisch, Heribert Sattel,
  Theo Gasser, and Ursula Schreiter-Gasser.
\newblock Eeg coherence in alzheimer disease.
\newblock \emph{Electroencephalography and clinical neurophysiology},
  90\penalty0 (3):\penalty0 242--245, 1994.

\bibitem[Bodnar et~al.(2022)Bodnar, Giovanni, Chamberlain, Liò, and
  Bronstein]{Bodnar2022}
Cristian Bodnar, Francesco~Di Giovanni, Benjamin~Paul Chamberlain, Pietro Liò,
  and Michael~M. Bronstein.
\newblock Neural sheaf diffusion: A topological perspective on heterophily and
  oversmoothing in {GNN}s.
\newblock In Alice~H. Oh, Alekh Agarwal, Danielle Belgrave, and Kyunghyun Cho
  (eds.), \emph{Advances in Neural Information Processing Systems}, 2022.

\bibitem[Borovitskiy et~al.(2020)Borovitskiy, Terenin, Mostowsky, and
  Deisenroth]{Borovitskiy2020}
Viacheslav Borovitskiy, Alexander Terenin, Peter Mostowsky, and Marc
  Deisenroth.
\newblock Mat\'{e}rn gaussian processes on riemannian manifolds.
\newblock In H.~Larochelle, M.~Ranzato, R.~Hadsell, M.F. Balcan, and H.~Lin
  (eds.), \emph{Advances in Neural Information Processing Systems}, volume~33,
  pp.\  12426--12437. Curran Associates, Inc., 2020.

\bibitem[Borovitskiy et~al.(2021)Borovitskiy, Azangulov, Terenin, Mostowsky,
  Deisenroth, and Durrande]{Borovitskiy2021}
Viacheslav Borovitskiy, Iskander Azangulov, Alexander Terenin, Peter Mostowsky,
  Marc Deisenroth, and Nicolas Durrande.
\newblock Mat{é}rn gaussian processes on graphs.
\newblock In Arindam Banerjee and Kenji Fukumizu (eds.), \emph{Proceedings of
  The 24th International Conference on Artificial Intelligence and Statistics},
  volume 130 of \emph{Proceedings of Machine Learning Research}, pp.\
  2593--2601. PMLR, 13--15 Apr 2021.

\bibitem[Bronstein et~al.(2017)Bronstein, Bruna, Lecun, Szlam, and
  Vandergheynst]{Bronstein2017}
Michael~M. Bronstein, Joan Bruna, Yann Lecun, Arthur Szlam, and Pierre
  Vandergheynst.
\newblock {Geometric Deep Learning: Going beyond Euclidean data}.
\newblock \emph{IEEE Signal Process. Mag.}, 34\penalty0 (4):\penalty0 18--42,
  2017.
\newblock ISSN 10535888.
\newblock \doi{10.1109/MSP.2017.2693418}.

\bibitem[Budninskiy et~al.(2019)Budninskiy, Yin, Feng, Tong, and
  Desbrun]{Budninskiy}
Max Budninskiy, Gloria Yin, Leman Feng, Yiying Tong, and Mathieu Desbrun.
\newblock Parallel transport unfolding: A connection-based manifold learning
  approach.
\newblock \emph{SIAM Journal on Applied Algebra and Geometry}, 3\penalty0
  (2):\penalty0 266--291, 2019.
\newblock \doi{10.1137/18M1196133}.

\bibitem[Chu(2015)]{chu2015high}
Catherine~J Chu.
\newblock High density eeg—what do we have to lose?
\newblock \emph{Clinical neurophysiology: official journal of the International
  Federation of Clinical Neurophysiology}, 126\penalty0 (3):\penalty0 433,
  2015.

\bibitem[Chung(1997)]{Chung1997}
Fan Chung.
\newblock \emph{{Spectral Graph Theocy}}, volume~92 of \emph{American
  Mathematical Soc.}
\newblock American Mathematical Soc., 1997.
\newblock ISBN 0821803158.

\bibitem[Coifman et~al.(2005)Coifman, Lafon, Lee, Maggioni, Nadler, Warner, and
  Zucker]{Coifman2005}
Ronald~R Coifman, Stéphane Lafon, Anne~B Lee, Mauro Maggioni, Boaz Nadler,
  Frederick Warner, and Steven~W Zucker.
\newblock {Geometric diffusions as a tool for harmonic analysis and structure
  definition of data: Diffusion maps}.
\newblock \emph{Proc. Natl. Acad. Sci. U. S. A.}, 102\penalty0 (21):\penalty0
  7426--7431, 2005.
\newblock \doi{10.1073/pnas.0500334102}.

\bibitem[Dauwels et~al.(2010)Dauwels, Vialatte, and
  Cichocki]{dauwels2010diagnosis}
Justin Dauwels, Francois Vialatte, and Andrzej Cichocki.
\newblock Diagnosis of alzheimer's disease from eeg signals: where are we
  standing?
\newblock \emph{Current Alzheimer Research}, 7\penalty0 (6):\penalty0 487--505,
  2010.

\bibitem[Defferrard et~al.(2016)Defferrard, Bresson, and
  Vandergheynst]{Defferrard2016}
Michaël Defferrard, Xavier Bresson, and Pierre Vandergheynst.
\newblock {Convolutional Neural Networks on Graphs with}.
\newblock In \emph{NIPS' 2016}, pp.\  3844--3852, 2016.
\newblock ISBN 9781510838819.

\bibitem[Delorme \& Makeig(2004)Delorme and Makeig]{delorme2004eeglab}
Arnaud Delorme and Scott Makeig.
\newblock Eeglab: an open source toolbox for analysis of single-trial eeg
  dynamics including independent component analysis.
\newblock \emph{Journal of neuroscience methods}, 134\penalty0 (1):\penalty0
  9--21, 2004.

\bibitem[Duncker \& Sahani(2018)Duncker and Sahani]{Duncker2018}
Lea Duncker and Maneesh Sahani.
\newblock {Temporal alignment and latent Gaussian process factor inference in
  population spike trains}.
\newblock \emph{Adv. Neural Inf. Process. Syst.}, 2018-December\penalty0
  (NeurIPS):\penalty0 10445--10455, 2018.
\newblock ISSN 10495258.

\bibitem[Fefferman et~al.(2016)Fefferman, Mitter, and
  Narayanan]{fefferman2016testing}
Charles Fefferman, Sanjoy Mitter, and Hariharan Narayanan.
\newblock Testing the manifold hypothesis.
\newblock \emph{Journal of the American Mathematical Society}, 29\penalty0
  (4):\penalty0 983--1049, 2016.

\bibitem[Gardner et~al.(2022)Gardner, Hermansen, Pachitariu, Burak, Baas, Dunn,
  Moser, and Moser]{Gardner2022}
Richard~J. Gardner, Erik Hermansen, Marius Pachitariu, Yoram Burak, Nils~A.
  Baas, Benjamin~A. Dunn, May~Britt Moser, and Edvard~I. Moser.
\newblock {Toroidal topology of population activity in grid cells}.
\newblock \emph{Nature}, 602\penalty0 (7895):\penalty0 123--128, 2022.
\newblock \doi{10.1038/s41586-021-04268-7}.

\bibitem[Gosztolai \& Arnaudon(2021)Gosztolai and Arnaudon]{Gosztolai2021}
Adam Gosztolai and Alexis Arnaudon.
\newblock {Unfolding the multiscale structure of networks with dynamical
  Ollivier-Ricci curvature}.
\newblock \emph{Nat. Commun.}, 12\penalty0 (1):\penalty0 1--11, 2021.
\newblock ISSN 20411723.
\newblock \doi{10.1038/s41467-021-24884-1}.

\bibitem[Gosztolai et~al.(2021)Gosztolai, G{\"{u}}nel, Lobato-R{\'{i}}os,
  {Pietro Abrate}, Morales, Rhodin, Fua, and Ramdya]{Gosztolai2021b}
Adam Gosztolai, Semih G{\"{u}}nel, Victor Lobato-R{\'{i}}os, Marco {Pietro
  Abrate}, Daniel Morales, Helge Rhodin, Pascal Fua, and Pavan Ramdya.
\newblock {LiftPose3D, a deep learning-based approach for transforming
  two-dimensional to three-dimensional poses in laboratory animals}.
\newblock \emph{Nat. Methods}, 18\penalty0 (8):\penalty0 975--981, 2021.
\newblock ISSN 1548-7091.
\newblock \doi{10.1038/s41592-021-01226-z}.

\bibitem[Gosztolai et~al.(2023)Gosztolai, Peach, Arnaudon, Barahona, and
  Vandergheynst]{Gosztolai2023}
Adam Gosztolai, Robert~L. Peach, Alexis Arnaudon, Mauricio Barahona, and Pierre
  Vandergheynst.
\newblock {Interpretable statistical representations of neural population
  dynamics and geometry}.
\newblock \emph{arXiv:2304.03376}, 2023.

\bibitem[Grattarola \& Vandergheynst(2022)Grattarola and
  Vandergheynst]{grattarola2022}
Daniele Grattarola and Pierre Vandergheynst.
\newblock Generalised implicit neural representations.
\newblock \emph{Advances in Neural Information Processing Systems},
  35:\penalty0 30446--30458, 2022.

\bibitem[Hutchinson et~al.(2021)Hutchinson, Terenin, Borovitskiy, Takao, Teh,
  and Deisenroth]{Hutchinson2021}
Michael Hutchinson, Alexander Terenin, Viacheslav Borovitskiy, So~Takao, Yee
  Teh, and Marc Deisenroth.
\newblock Vector-valued gaussian processes on riemannian manifolds via gauge
  independent projected kernels.
\newblock In M.~Ranzato, A.~Beygelzimer, Y.~Dauphin, P.S. Liang, and J.~Wortman
  Vaughan (eds.), \emph{Advances in Neural Information Processing Systems},
  volume~34, pp.\  17160--17169. Curran Associates, Inc., 2021.

\bibitem[Illoul \& Lorong(2011)Illoul and Lorong]{illoul2011some}
Lounes Illoul and Philippe Lorong.
\newblock On some aspects of the cnem implementation in 3d in order to simulate
  high speed machining or shearing.
\newblock \emph{Computers \& Structures}, 89\penalty0 (11-12):\penalty0
  940--958, 2011.

\bibitem[Jensen et~al.(2020)Jensen, Kao, Tripodi, and Hennequin]{Jensen2020}
Kristopher~T. Jensen, Ta~Chu Kao, Marco Tripodi, and Guillaume Hennequin.
\newblock {Manifold GPLVMs for discovering non-Euclidean latent structure in
  neural data}.
\newblock \emph{Adv. Neural Inf. Process. Syst.}, 2020-Decem:\penalty0 1--22,
  2020.
\newblock ISSN 10495258.

\bibitem[{Kabsch}(1976)]{kabsch}
Wolfgang {Kabsch}.
\newblock {A solution for the best rotation to relate two sets of vectors}.
\newblock \emph{Acta Crystallographica Section A}, 32\penalty0 (5):\penalty0
  922--923, September 1976.
\newblock \doi{10.1107/S0567739476001873}.

\bibitem[Khona \& Fiete(2022)Khona and Fiete]{Khona2022}
Mikail Khona and Ila~R. Fiete.
\newblock {Attractor and integrator networks in the brain}.
\newblock \emph{Nat. Rev. Neurosci.}, 23\penalty0 (12):\penalty0 744--766,
  2022.
\newblock \doi{10.1038/s41583-022-00642-0}.

\bibitem[Kipf \& Welling(2017)Kipf and Welling]{Kipf2017}
Thomas~N. Kipf and Max Welling.
\newblock {Semi-Supervised Classification with Graph Convolutional Networks}.
\newblock \emph{ICLR}, 2017.
\newblock ISSN 10963626.
\newblock URL \url{arXiv.org}.

\bibitem[Kn{\"{o}}ppel et~al.(2013)Kn{\"{o}}ppel, Crane, Pinkall, and
  Schr{\"{o}}der]{Knoppel2013}
Felix Kn{\"{o}}ppel, Keenan Crane, Ulrich Pinkall, and Peter Schr{\"{o}}der.
\newblock {Globally optimal direction fields}.
\newblock \emph{ACM Trans. Graph.}, 32\penalty0 (4), 2013.
\newblock \doi{10.1145/2461912.2462005}.

\bibitem[Kn{\"{o}}ppel et~al.(2015)Kn{\"{o}}ppel, Crane, Pinkall, and
  Schr{\"{o}}der]{Knoppel2015}
Felix Kn{\"{o}}ppel, Keenan Crane, Ulrich Pinkall, and Peter Schr{\"{o}}der.
\newblock {Stripe patterns on surfaces}.
\newblock \emph{ACM Trans. Graph.}, 34\penalty0 (4), 2015.
\newblock ISSN 15577368.
\newblock \doi{10.1145/2767000}.

\bibitem[Koestler et~al.(2022)Koestler, Grittner, Moeller, Cremers, and
  L{\"{a}}hner]{Koestler2022}
Lukas Koestler, Daniel Grittner, Michael Moeller, Daniel Cremers, and Zorah
  L{\"{a}}hner.
\newblock {Intrinsic Neural Fields: Learning Functions on Manifolds}.
\newblock \emph{Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif.
  Intell. Lect. Notes Bioinformatics)}, 13662 LNCS:\penalty0 622--639, 2022.
\newblock ISSN 16113349.
\newblock \doi{10.1007/978-3-031-20086-1_36}.

\bibitem[{La Manno} et~al.(2018){La Manno}, Soldatov, Zeisel, Braun,
  Hochgerner, Petukhov, Lidschreiber, Kastriti, L{\"{o}}nnerberg, Furlan, Fan,
  Borm, Liu, van Bruggen, Guo, He, Barker, Sundstr{\"{o}}m, Castelo-Branco,
  Cramer, Adameyko, Linnarsson, and Kharchenko]{LaManno2018}
Gioele {La Manno}, Ruslan Soldatov, Amit Zeisel, Emelie Braun, Hannah
  Hochgerner, Viktor Petukhov, Katja Lidschreiber, Maria~E. Kastriti, Peter
  L{\"{o}}nnerberg, Alessandro Furlan, Jean Fan, Lars~E. Borm, Zehua Liu, David
  van Bruggen, Jimin Guo, Xiaoling He, Roger Barker, Erik Sundstr{\"{o}}m,
  Gon{\c{c}}alo Castelo-Branco, Patrick Cramer, Igor Adameyko, Sten Linnarsson,
  and Peter~V. Kharchenko.
\newblock {RNA velocity of single cells}.
\newblock \emph{Nature}, 560\penalty0 (7719):\penalty0 494--498, 2018.
\newblock ISSN 14764687.
\newblock \doi{10.1038/s41586-018-0414-6}.

\bibitem[Lipman(2021)]{Lipman2021}
Yaron Lipman.
\newblock {Phase Transitions, Distance Functions, and Implicit Neural
  Representations}.
\newblock \emph{Proc. Mach. Learn. Res.}, 139:\penalty0 6702--6712, 2021.
\newblock ISSN 26403498.

\bibitem[Mallasto \& Feragen(2018)Mallasto and Feragen]{Mallasto2018}
Anton Mallasto and Aasa Feragen.
\newblock Wrapped gaussian process regression on riemannian manifolds.
\newblock In \emph{Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition (CVPR)}, June 2018.

\bibitem[Mallasto et~al.(2020)Mallasto, Hauberg, and Feragen]{Mallasto2020}
Anton Mallasto, S{\o}ren Hauberg, and Aasa Feragen.
\newblock {Probabilistic Riemannian submanifold learning with wrapped Gaussian
  process latent variable models}.
\newblock \emph{AISTATS 2019 - 22nd Int. Conf. Artif. Intell. Stat.}, 89, 2020.

\bibitem[Mildenhall et~al.(2020)Mildenhall, Srinivasan, Tancik, Barron,
  Ramamoorthi, and Ng]{Mildenhall2022}
Ben Mildenhall, Pratul~P. Srinivasan, Matthew Tancik, Jonathan~T. Barron, Ravi
  Ramamoorthi, and Ren Ng.
\newblock Nerf: Representing scenes as neural radiance fields for view
  synthesis.
\newblock In \emph{ECCV}, 2020.

\bibitem[Moretti et~al.(2004)Moretti, Babiloni, Binetti, Cassetta, Dal~Forno,
  Ferreric, Ferri, Lanuzza, Miniussi, Nobili, et~al.]{moretti2004individual}
Davide~V Moretti, Claudio Babiloni, Giuliano Binetti, Emanuele Cassetta, Gloria
  Dal~Forno, Florinda Ferreric, Raffaele Ferri, Bartolo Lanuzza, Carlo
  Miniussi, Flavio Nobili, et~al.
\newblock Individual analysis of eeg frequency and band power in mild
  alzheimer's disease.
\newblock \emph{Clinical Neurophysiology}, 115\penalty0 (2):\penalty0 299--308,
  2004.

\bibitem[Ortega et~al.(2018)Ortega, Frossard, Kovacevic, Moura, and
  Vandergheynst]{Ortega}
Antonio Ortega, Pascal Frossard, Jelena Kovacevic, Jose~M.F. Moura, and Pierre
  Vandergheynst.
\newblock {Graph Signal Processing: Overview, Challenges, and Applications}.
\newblock \emph{Proc. IEEE}, 106\penalty0 (5):\penalty0 808--828, 2018.
\newblock ISSN 15582256.
\newblock \doi{10.1109/JPROC.2018.2820126}.

\bibitem[Peach et~al.(2020)Peach, Arnaudon, and Barahona]{peach2020semi}
Robert~L Peach, Alexis Arnaudon, and Mauricio Barahona.
\newblock Semi-supervised classification on graphs using explicit diffusion
  dynamics.
\newblock \emph{Foundations of Data Science}, 2\penalty0 (1):\penalty0 19--33,
  2020.

\bibitem[Perrin et~al.(1989)Perrin, Pernier, Bertrand, and
  Echallier]{perrin1989spherical}
Fran{\c{c}}ois Perrin, Jacques Pernier, Olivier Bertrand, and Jean~Francois
  Echallier.
\newblock Spherical splines for scalp potential and current density mapping.
\newblock \emph{Electroencephalography and clinical neurophysiology},
  72\penalty0 (2):\penalty0 184--187, 1989.

\bibitem[Qi et~al.(2017)Qi, Su, Mo, and Guibas]{Qi2017}
Charles~R. Qi, Hao Su, Kaichun Mo, and Leonidas~J. Guibas.
\newblock {PointNet: Deep learning on point sets for 3D classification and
  segmentation}.
\newblock \emph{Proc. - 30th IEEE Conf. Comput. Vis. Pattern Recognition, CVPR
  2017}, 2017-January:\penalty0 77--85, 2017.
\newblock \doi{10.1109/CVPR.2017.16}.

\bibitem[Rasmussen \& Williams(2006)Rasmussen and Williams]{Rasmussen2006}
Carl~Edward Rasmussen and Christopher K.~I. Williams.
\newblock \emph{{Gaussian Processes for Machine Learning}}.
\newblock MIT press, 2006.
\newblock ISBN 026218253X.

\bibitem[Roberts et~al.(2019)Roberts, Gollo, Abeysuriya, Roberts, Mitchell,
  Woolrich, and Breakspear]{roberts2019metastable}
James~A Roberts, Leonardo~L Gollo, Romesh~G Abeysuriya, Gloria Roberts,
  Philip~B Mitchell, Mark~W Woolrich, and Michael Breakspear.
\newblock Metastable brain waves.
\newblock \emph{Nature communications}, 10\penalty0 (1):\penalty0 1056, 2019.

\bibitem[Robinson et~al.(2017)Robinson, Venkatesh, Boring, Tarr, Grover, and
  Behrmann]{robinson2017very}
Amanda~K Robinson, Praveen Venkatesh, Matthew~J Boring, Michael~J Tarr, Pulkit
  Grover, and Marlene Behrmann.
\newblock Very high density eeg elucidates spatiotemporal aspects of early
  visual processing.
\newblock \emph{Scientific reports}, 7\penalty0 (1):\penalty0 16248, 2017.

\bibitem[Sato et~al.(2012)Sato, Nauhaus, and Carandini]{sato2012traveling}
Tatsuo~K Sato, Ian Nauhaus, and Matteo Carandini.
\newblock Traveling waves in visual cortex.
\newblock \emph{Neuron}, 75\penalty0 (2):\penalty0 218--229, 2012.

\bibitem[Seeber et~al.(2019)Seeber, Cantonas, Hoevels, Sesia,
  Visser-Vandewalle, and Michel]{seeber2019subcortical}
Martin Seeber, Lucia-Manuela Cantonas, Mauritius Hoevels, Thibaut Sesia, Veerle
  Visser-Vandewalle, and Christoph~M Michel.
\newblock Subcortical electrophysiological activity is detectable with
  high-density eeg source imaging.
\newblock \emph{Nature communications}, 10\penalty0 (1):\penalty0 753, 2019.

\bibitem[Sharp et~al.(2019)Sharp, Soliman, and Crane]{Sharp2019}
Nicholas Sharp, Yousuf Soliman, and Keenan Crane.
\newblock {The vector heat method}.
\newblock \emph{ACM Trans. Graph.}, 38\penalty0 (3), 2019.
\newblock \doi{10.1145/3243651}.

\bibitem[Siclari et~al.(2018)Siclari, Bernardi, Cataldi, and
  Tononi]{siclari2018dreaming}
Francesca Siclari, Giulio Bernardi, Jacinthe Cataldi, and Giulio Tononi.
\newblock Dreaming in nrem sleep: a high-density eeg study of slow waves and
  spindles.
\newblock \emph{Journal of Neuroscience}, 38\penalty0 (43):\penalty0
  9175--9185, 2018.

\bibitem[Singer \& Wu(2012)Singer and Wu]{Singer2012}
Amit Singer and Hau~Tieng Wu.
\newblock {Vector diffusion maps and the connection Laplacian}.
\newblock \emph{Commun. Pure Appl. Math.}, 65\penalty0 (8):\penalty0
  1067--1144, 2012.
\newblock \doi{10.1002/cpa.21395}.

\bibitem[Singer \& Wu(2017)Singer and Wu]{Singer2017}
Amit Singer and Hau~Tieng Wu.
\newblock {Spectral convergence of the connection Laplacian from random
  samples}.
\newblock \emph{Inf. Inference}, 6\penalty0 (1):\penalty0 58--123, 2017.
\newblock \doi{10.1093/imaiai/iaw016}.

\bibitem[Sitzmann et~al.(2020)Sitzmann, Martel, Bergman, Lindell, and
  Wetzstein]{Sitzmann2020}
Vincent Sitzmann, Julien~N.P. Martel, Alexander~W. Bergman, David~B. Lindell,
  and Gordon Wetzstein.
\newblock {Implicit neural representations with periodic activation functions}.
\newblock \emph{Adv. Neural Inf. Process. Syst.}, 2020-December\penalty0
  (NeurIPS):\penalty0 1--12, 2020.
\newblock ISSN 10495258.

\bibitem[Solin \& S{\"{a}}rkk{\"{a}}(2020)Solin and
  S{\"{a}}rkk{\"{a}}]{Solin2020}
Arno Solin and Simo S{\"{a}}rkk{\"{a}}.
\newblock {Hilbert space methods for reduced-rank Gaussian process regression}.
\newblock \emph{Stat. Comput.}, 30\penalty0 (2):\penalty0 419--446, 2020.
\newblock ISSN 15731375.
\newblock \doi{10.1007/s11222-019-09886-w}.

\bibitem[Sussillo \& Barak(2013)Sussillo and Barak]{Sussillo2013}
David Sussillo and Omri Barak.
\newblock {Opening the black box: low-dimensional dynamics in high-dimensional
  recurrent neural networks}.
\newblock \emph{Neural Comput.}, 25\penalty0 (3):\penalty0 626--649, 2013.
\newblock \doi{10.1162/NECO_a_00409}.

\bibitem[Taubin(1995)]{taubin}
Gabriel Taubin.
\newblock A signal processing approach to fair surface design.
\newblock In \emph{Proceedings of the 22nd Annual Conference on Computer
  Graphics and Interactive Techniques}, SIGGRAPH '95, pp.\  351–358, New
  York, NY, USA, 1995. Association for Computing Machinery.
\newblock ISBN 0897917014.
\newblock \doi{10.1145/218380.218473}.

\bibitem[Tenenbaum(2000)]{Tenenbaum2000}
Joshua~B Tenenbaum.
\newblock {A Global Geometric Framework for Nonlinear Dimensionality
  Reduction}.
\newblock \emph{Science (80-. ).}, 290\penalty0 (5500):\penalty0 2319--2323,
  2000.
\newblock \doi{10.1126/science.290.5500.2319}.

\bibitem[Titsias(2009)]{titsias2009}
Michalis Titsias.
\newblock Variational learning of inducing variables in sparse gaussian
  processes.
\newblock In David van Dyk and Max Welling (eds.), \emph{Proceedings of the
  Twelth International Conference on Artificial Intelligence and Statistics},
  volume~5 of \emph{Proceedings of Machine Learning Research}, pp.\  567--574,
  Hilton Clearwater Beach Resort, Clearwater Beach, Florida USA, 16--18 Apr
  2009. PMLR.

\bibitem[Whittle(1963)]{Whittle1963}
Peter Whittle.
\newblock Stochastic-processes in several dimensions.
\newblock \emph{Bulletin of the International Statistical Institute},
  40\penalty0 (2):\penalty0 974--994, 1963.

\bibitem[Wilson et~al.(2021)Wilson, Borovitskiy, Terenin, Mostowsky, and
  Deisenroth]{Wilson2021}
James~T. Wilson, Viacheslav Borovitskiy, Alexander Terenin, Peter Mostowsky,
  and Marc~Peter Deisenroth.
\newblock {Pathwise conditioning of gaussian processes}.
\newblock \emph{J. Mach. Learn. Res.}, 22:\penalty0 1--47, 2021.

\bibitem[Xu et~al.(2023)Xu, Long, Feng, and Gong]{xu2023interacting}
Yiben Xu, Xian Long, Jianfeng Feng, and Pulin Gong.
\newblock Interacting spiral wave patterns underlie complex brain dynamics and
  are related to cognitive processing.
\newblock \emph{Nature Human Behaviour}, pp.\  1--20, 2023.

\bibitem[Yu et~al.(2009)Yu, Cunningham, Santhanam, Ryu, Shenoy, and
  Sahani]{Yu2009}
Byron~M. Yu, John~P. Cunningham, Gopal Santhanam, Stephen~I. Ryu, Krishna~V.
  Shenoy, and Maneesh Sahani.
\newblock {Gaussian-process factor analysis for low-dimensional single-trial
  analysis of neural population activity}.
\newblock \emph{J. Neurophysiol.}, 102\penalty0 (1):\penalty0 614--635, 2009.
\newblock ISSN 15221598.
\newblock \doi{10.1152/jn.90941.2008}.

\bibitem[Zetterberg \& Bendlin(2021)Zetterberg and
  Bendlin]{zetterberg2021biomarkers}
Henrik Zetterberg and Barbara~B Bendlin.
\newblock Biomarkers for alzheimer’s disease—preparing for a new era of
  disease-modifying therapies.
\newblock \emph{Molecular psychiatry}, 26\penalty0 (1):\penalty0 296--308,
  2021.

\end{thebibliography}

